Latent variable modeling with random features

Gaussian process-based latent variable models are flexible and theoretically grounded tools for nonlinear dimension reduction, but generalizing to non-Gaussian data likelihoods within this nonlinear framework is statistically challenging. Here, we use random features to develop a family of nonlinear dimension reduction models that are easily extensible to non-Gaussian data likelihoods; we call these random feature latent variable models (RFLVMs). By approximating a nonlinear relationship between the latent space and the observations with a function that is linear with respect to random features, we induce closed-form gradients of the posterior distribution with respect to the latent variable. This allows the RFLVM framework to support computationally tractable nonlinear latent variable models for a variety of data likelihoods in the exponential family without specialized derivations. Our generalized RFLVMs produce results comparable with other state-of-the-art dimension reduction methods on diverse types of data, including neural spike train recordings, images, and text data.

==> 5_impact.tex <==
% https://medium.com/@NeurIPSConf/a-note-for-submitting-authors-48cebfebae82

% "Use unnumbered first level headings for this section, which should go at the end of the paper. Note tthat this section does not count towards the eight pages of content that are allowed."

% "This year we are asking all authors to include a broader impact section to their paper (included in the new paper template). This section does not count towards the 8-page limit, and it should go before the references. It should include a statement about the foreseeable positive impact as well as potential risks and associated mitigations of the proposed research. We expect authors to write about two paragraphs, minimizing broad speculations. Authors can also declare that a broader impact statement is not applicable to their work, if they believe it to be the case. Reviewers will be asked to review papers on the basis of technical merit. Reviewers will also confirm whether the broader impact section is adequate, but this assessment will not affect the overall rating. However, reviewers will also have the option to flag a paper for ethical concerns, which may relate to the content of the broader impact section. If such concerns are shared by the Area Chair and Senior Area Chair, the paper will be sent for additional review to a pool of emergency reviewers with expertise in Machine Learning and Ethics, who will provide an assessment solely on the basis of ethical considerations. Program Chairs will then review each such case, aggregate all the feedback and make a final decision on the paper. We expect very few, if any, papers to need such further assessment. More information is available in the FAQ."

\section*{Broader Impact}
%Dimension reduction is an important task in data analysis, particularly in many scientific fields such as biology, neuroscience, and the social sciences. The line of research goes back over a century \citep{pearson1901liii}.
Dimension reduction an important task in many scientific fields such as biology, neuroscience, and the social sciences, enabling scientists to discover patterns in data and then to articulate and test hypotheses based on those findings. For example, the data collection process often introduces biases, and dimension reduction is a first step in detecting such problems. We acknowledge that dimension reduction, like any other tool, can be used unethically by bad actors, and therefore we stress the importance of building simple, accessible, and interpretable dimension reduction models. Gaussian process-based latent variable models are appealing because the methods are mathematically well-understood; inference is relatively cheap, requiring less compute than other sophisticated methods; and the inferred parameters have established meanings in statistics.


% . We see no ethical issues that are inherent to our work and no immediate connections to broader concerns such as human rights, privacy, job loss, bias, inclusion, or safety \citep{jobin2019global}. One benefit of our approach is that it facilitates inference for latent variable models, in terms of tractability and computational effort compared to other sophisticated state-of-the-art methods. This benefit democratizes the use of such models, without requiring intense cloud computing resources. However, the downside of democratizing machine learning is the risk of empowering unintended and unethical applications (for example, using deep learning methods to generate ``deepfakes''). \michael{Is there anything we can really do to stop bad behavior once the idea and code are public?}

% \michael{TODO: Find a nice way to thread in next paragraph nicely with the previous paragraph}
% To the contrary, principled and interpretable latent variable modeling plays an important role in scientific data analysis. These techniques are particularly useful for data in which the significance of the observations is not well-understood. For example, manifold learning is popular in computational neuroscience because modern neuroscientists can now simultaneously measure the activity of thousands of neurons without necessarily understanding what computations those neurons are performing \citep{saxena2019towards}. For these types of problems, interpretable dimension reduction is an important part of the scientific process.



% you might modify the statement to read something like: The goal of dimension reduction is to explore patterns underlying data; to this end, our model, to the extent to which it captures these patterns well in data types that often confound Gaussian models, may allow the identification and elucidation of patterns of bias in existing data sets.
% you might also add that the inference is (relatively) fast, meaning that you don't have to be a billionaire to run it and melt a whole city doing that.

==> _archive_2_background.tex <==
\section{Background}\label{sec:related}

\greg{also \url{https://papers.nips.cc/paper/4588-nystrom-method-vs-random-fourier-features-a-theoretical-and-empirical-comparison.pdf}}

% Random Fourier features are a popular method to scale kernel machines and have been used in kernel ridge regression \citep{avron2017random}, variational inference of GPs \citep{hensman2017variational} and sparse-spectrum GPs \cite{lazaro2010sparse}

\subsection{Dimension Reduction}

% PCA is a standard method for dimensionality reduction. Suppose we observe data $\smash{\Y = [\y_1 \dots \y_N]^{\top}}$, having $N$ samples and $J$ dimensions. We want to project $\Y$ to a $D \ll J$ dimensional representation $\smash{\X = [\x_1 \dots \x_N]^{\top}}$ such that maximum variance in $\Y$ is preserved in $\X$. The optimal linear projection for PCA are the $D$ right singular vectors corresponding to the $D$ largest eigenvalues of the covariance matrix of $\Y$ after mean centering. Two probabilistic formulations are probabilistic PCA \citep{tipping1999probabilistic} and dual probabilistic PCA \citep{lawrence2005probabilistic}, both which model the data as
% %
% \begin{equation}
%     \y_j \sim \N_{N}(\X \bbeta_j, \sigma_{Y}^{2} \eye),
%     \qquad
%     \bbeta_j \sim \mathcal{N}_{D}(0, \sigma_{\beta}^{2} \eye),
%     \qquad
%     \x_n \sim \N_D(\zero, \eye).
% \end{equation}
% %
% Probabilistic PCA marginalizes out $\X$ and optimizes the marginal likelihood with respect to $\bbeta_j$. Dual probabilistic PCA marginalizes out $\bbeta_j$ and optimizes the marginal likelihood with respect $\X$. For both methods, the maximum likelihood estimate is equivalent to the variance-preserving solution of PCA \citep{lawrence2004gaussian}.

PCA is a standard method for dimension reduction. Suppose we observe data $\smash{\Y = [\y_1 \dots \y_N]^{\top}}$, having $N$ samples and $J$ dimensions. We want to project $\Y$ to a $D \ll J$ dimensional representation $\smash{\X = [\x_1 \dots \x_N]^{\top}}$ such that maximum variance in $\Y$ is preserved in $\X$ \citep{hotelling1933analysis}. Probabilistic PCA \citep{roweis1998algorithms,tipping1999probabilistic, lawrence2005probabilistic} interprets PCA as a latent variable model with $J$ linear maps from latent to observation space, and the maximum likelihood estimate is equivalent to the variance-preserving solution of PCA \citep{lawrence2004gaussian}.

For a nonlinear model, a typical assumption is that the mapping between $\X$ and $\Y$ is GP-distributed. GPs are commonly used as priors over the space of arbitrary real-valued functions. This leads to the Gaussian process latent variable model \citep{lawrence2004gaussian}. %A Gaussian process becomes multivariate normal distributed at a finite collection of points, evaluated at its mean and covariance functions.
% this sentence is not useful. I'd remove. What is the goal of this paragraph? to describe GPs or GPLVMs? I think the latter. See sentence below:
A GPLVM uses Gaussian processes to create an arbitrary nonlinear map of a latent space $\X$ onto the noiseless observations $f_j(\X)$.
If we take the mean function to be zero, a GPLVM has the form:
%
\begin{equation}
\y_j \sim \N_N(f_{j}(\X), \sigma^{2}_Y \eye),
\quad
f_{j}(\X) \sim \N_N(\zero, \K_X),
\quad
\x_n \sim \N_{D}(\zero, \eye),
\label{eq:gplvm_def}
\end{equation}
%
where $\K_X$ is an $N \times N$ covariance kernel defined by a positive definite kernel function $k(\x, \xp)$ and $\smash{f_j(\X) = [f_{j}(\x_1) \dots f_{j}(\x_N)]^{\top}}$. Due to conjugacy between the GP and Gaussian likelihood, we can integrate out the noiseless observations $f_{j}(\X)$  in closed form. The resulting marginal likelihood for $\y_j$ is $\smash{\N_{N}(0, \K_{X} + \sigma^{2}_{j} \eye)}$. Despite this closed form distribution, we cannot obtain the optimal $\X$ analytically, but various approximations have been proposed. For example, a maximum a posteriori (MAP) estimation optimizes the marginal likelihood with respect to $\X$ using scaled conjugate gradients~\citep{lawrence2004gaussian,lawrence2005probabilistic}. Alternatively, \cite{titsias2010bayesian} derive a variational lower bound to the marginal likelihood for a variational approximation of the posterior of $\X$.

% And \cite{damianou2016variational} extend this variational result to the cases where the latent space exhibits time dependence, as well as to nonlinear state-space models.

% GP methods typically scale $O(N^3)$ with respect to the number of observations, due to the computational costs of inverting the covariance matrix. Nystr\"{o}m kernel approximations are popular in GP modeling to reduce this cubic computational costs. Sparse GPs methods \citep[for example]{snelson2006sparse} form a Nystr\"{o}m approximation of the covariance kernel, by learning a set of $ M \ll N $ ``inducing points'' which represent the input data and form the low-rank decomposition of the covariance kernel into $ N\times M $ and $ M \times M $ matrices, thereby reducing the computational complexity of fitting such models to $O(NM^{2})$. 

% not clear how this paragraph follows from the one above.
The computational complexity of GP methods is $O(N^3)$ due to matrix inversions. GPLVMs have incorporated sparse GP approximations 
% what is a 'sparse GP approach? i think you mean something different.
such as Nystr\"{o}m kernel approximations \citep[for example]{snelson2006sparse} to reduce this complexity and 
% change the wording of the next phrase - say it without "dependence"
the tight dependence between $\smash{\F = [f_1(\X) \dots f_J(\X)]^{\top}}$ and $\X$ \citep{titsias2010bayesian,damianou2016variational}. However, sparse methods prune support for the relationship between $\X $ and $\F$, but do not fundamentally change its complexity.  Sparse GPLVM approximations still rely on Gaussian conjugacy to marginalize $\F$ and optimize $\X$.
% above we say that marginalizing out F doesn't easily allow optimization of X, so this statement isn't clear.
Moreover, sparse approximations require using an ARD-RBF kernel to compute the variational lower bound of the marginal likelihood analytically, which restricts the generalizability of such methods to only specific modeling scenarios. % is this true? all sparse approximations? I'm not really sure this is true, nor do i see the the point of this statement.

\cite{wu2017gaussian} addresses this problem for Poisson likelihoods using a decoupled Laplace approximation to iteratively approximate marginalizing out $\F$ and then taking a MAP estimate of $\X$. However, this approach works by approximating a Poisson likelihood with a Gaussian, and it is not general to a wider class of likelihoods.  \cite{gal2015latent} introduced a GP-LVM model for multinomial likelihoods, however, they develop a variational approximation tailored specifically for the multinomial distribution.

%Typical gradient-based methods %Markov chain Monte Carlo (MCMC) methods for sampling the posterior of $\X$, like Hamiltonian Monte Carlo (HMC) or optimization-based methods like the Laplace approximation, can quickly be trapped in sub-optimal local modes due to this tight coupling.
 
%Their method partially breaks the dependence between $\f_j$ and $\X$.  Given the desired posterior $p(\f_j \mid \y_j, \X) \propto p(\y_j \mid \f_j) p(\f_j \mid \X)$, they perform a standard Laplace approximation of the $p(\f_j \mid \y_j, \X)$ with a second-order Taylor expansion and then they approximate the Poisson likelihood as a Gaussian distribution, $\N_N(\m, \S)$. The relationship between the two Gaussian distributions allows them to analytically solve for $\m$ and $\S$ and obtain a MAP estimate for $\X$.

Each of the aforementioned GPLVM methods are tailored for a specific likelihood. Without marginalizing the mapping functions $\F$, learning $\X$  becomes especially hard with optimization due to the dependence between $ \F$ and $\X$ (which we will demonstrate in Section~\ref{sec:method}). Thus, inference still remains challenging for non-Gaussian data.

\subsection{Random Kernel Approximations}

We propose breaking the strong dependency between $\F$ and $\X$ by approximating the GP-distributed maps using random Fourier features \citep[][RFFs]{rahimi2008random}. Bochner's theorem \citep{bochner1959lectures} states that any continuous shift-invariant kernel $k(\x, \xp) = k(\x - \xp)$ on $\Reals^D$ is positive definite if and only if $k(\x - \xp)$ is the Fourier transform of a non-negative measure $p(\w)$. If the kernel is properly scaled, the kernel's Fourier transform $p(\w)$ is guaranteed to be a density. Let $\smash{h(\x) \triangleq \exp(i \w^{\top} \x)}$ and let $h(\x)^{*}$ denotes its complex conjugate, and then observe that
%
\begin{equation}
k(\x - \xp)
=
\int_{\Reals^D} p(\w) \exp(i \w^{\top} (\x - \xp)) \d\w
=
\E_{p(\w)}[h(\x)h(\x)^{*}].
\label{eq:rffs_mc_int}
\end{equation}
%
So $h(\x)h(\x)^{*}$ is an unbiased estimate of $k(\x - \xp)$. If we drop the imaginary part for real-valued kernels, we can re-define $\smash{h(\x) \triangleq \cos(\w^{\top}\x)}$ by Euler's formula and then use Monte Carlo integration to approximate \eqref{eq:rffs_mc_int} as $\smash{\varphi(\x)^{\top} \varphi(\x)}$ where
%
\begin{equation}
    \varphi(\x) \triangleq \sqrt{\frac{2}{M}} \begin{bmatrix}
    \sin(\w_1^{\top} \x) & \cos(\w_1^{\top} \x) & \dots & \sin(\w_{M/2}^{\top} \x) & \cos(\w_{M/2}^{\top} \x)
    \end{bmatrix}^{\top}
\label{eq:rff_def}
\end{equation}
%
and where $\smash{\w_m \stackrel{\texttt{iid}}{\sim} p(\w)}$. See Appendix~\ref{app:rff_correctness} for details on correctness. The benefit of \eqref{eq:rff_def} is that a representer theorem \citep{kimeldorf1971some} tells us that the optimal solution $f^{*}(\x)$ for kernel methods is a weighted function of the kernel evaluated at the observations, giving us
%
\begin{equation}
f^{*}(\x)
= \sum_{n=1}^{N} \alpha_n k(\x_n, \x)
= \sum_{n=1}^{N} \alpha_n \langle \phi(\x_n), \phi(\x) \rangle_{\mathcal{V}}
\approx \sum_{n=1}^{N} \alpha_n \varphi(\x_n)^{\top} \varphi(\x)
= \bbeta^{\top} \varphi(\x).
\label{eq:kernel_approx}
\end{equation}
%
In the second equality in \eqref{eq:kernel_approx}, the kernel trick implicitly lifts the data into a Reproducing Kernel Hilbert Space $\mathcal{V}$ in which the optimal solution is a linear operator. RFFs approximates this inner product, allowing us to estimate the GP's nonlinear maps as linear in the random projection $\varphi(\x)$. The approximation converges exponentially fast in $M$ by Hoeffding's inequality and \cite{rahimi2008random} proved that the Fourier features converge uniformly.

\michael{TODO: Discussion about other factor models: Poisson factor analysis, NNMF, generalized PCA}

\subsection{Spectral Mixture Kernels}
RFFs are a popular technique to scale kernel methods. However, \cite{yang2012nystrom} show that a data-driven approach to learning $\W = [\w_1 \dots \w_{M/2}]^{\top}$, as opposed to \textit{i.i.d.} draws from $p(\w)$ used in \cite{rahimi2008random}, will more accurately approximate a covariance kernel. We can therefore use RFF approximations in a more effective Bayesian manner by assuming a prior distribution on $p(\w)$ and learning the posterior of $\w$. \cite{lazaro2010sparse} used an RFF approximation for scalable GP regression, and learned the random frequencies by optimizing the marginal likelihood. 

However, a crucial question here is which choice of covariance function to use? %At the same time, choosing a kernel in GP-based models and learning the kernel hyperparameters is crucial for the performance of the model. 
The radial basis function kernel, whose Fourier transform corresponds to is a spherical Gaussian, $p(\w)\sim \N_D (\mathbf{0}, \sigma^{2}\eye)$, 
%an RBF kernel with inverse length scale $\sigma^2$.
is a typical default option even though the true covariance function is usually unknown \textit{a priori}. A flexible alternative is to use a spectral mixture kernel. \cite{wilson2013gaussian} originally propose using a scale-mixture mixture of Gaussians as the spectral density, $p(\w)$, as they are a universal approximator for any continuous distribution. Therefore, its equivalent representation as a spectral mixture kernel can approximate any stationary covariance function.

\cite{oliva2016bayesian} extend the spectral mixture kernel from \cite{wilson2013gaussian} to a scalable Bayesian non-parametric kernel learning (BaNK) method by assuming $p(\w)$ is a Dirichlet process mixture of Gaussians\footnote{See \cite{ferguson1973bayesian, sethuraman1994constructive, aldous1985exchangeability} for details.} in order to adaptively learn the mixtures and by operating purely in the space of random features in order to apply the RFF approximation in Gaussian process models. By sampling the posterior space of $\W$, we can explore the space of stationary kernels which also allows us to evaluate the hyperparameters of the covariance kernel in a proper Bayesian manner.
